Infant hip screening using multi-class ultrasound scan segmentation

Developmental dysplasia of the hip (DDH) is a condition in infants where the femoral head is incorrectly located in the hip joint. We propose a deep learning algorithm for segmenting key structures within ultrasound images, employing this to calculate Femoral Head Coverage (FHC) and provide a screening diagnosis for DDH. To our knowledge, this is the first study to automate FHC calculation for DDH screening. Our algorithm outperforms the international state of the art, agreeing with expert clinicians on 89.8% of our test images.

==> 2023-images/ChangingDecisionValue/ChangedDecisionValueForFHC.tex <==
DECISION VALUE: 45
Correct FHC: 41 Incorrect FHC: 8 Accuracy: 0.8367346938775511
TRUE POSITIVE : 25
TRUE NEGATIVE : 16
FALSE POSITIVE : 1
FALSE NEGATIVE  : 7
TRUE POSITIVE RATE : 0.78125
TRUE NEGATIVE RATE : 0.9411764705882353
FALSE POSITIVE RATE : 0.058823529411764705
FALSE NEGATIVE RATE : 0.21875

DECISION VALUE: 50
Correct FHC: 44 Incorrect FHC: 5 Accuracy: 0.8979591836734694
TRUE POSITIVE : 29
TRUE NEGATIVE : 15
FALSE POSITIVE : 2
FALSE NEGATIVE  : 3
TRUE POSITIVE RATE : 0.90625
TRUE NEGATIVE RATE : 0.8823529411764706
FALSE POSITIVE RATE : 0.11764705882352941
FALSE NEGATIVE RATE : 0.09375

DECISION VALUE: 54
Correct FHC: 41 Incorrect FHC: 8 Accuracy: 0.8367346938775511
TRUE POSITIVE : 31
TRUE NEGATIVE : 10
FALSE POSITIVE : 7
FALSE NEGATIVE  : 1
TRUE POSITIVE RATE : 0.96875
TRUE NEGATIVE RATE : 0.5882352941176471
FALSE POSITIVE RATE : 0.4117647058823529
FALSE NEGATIVE RATE : 0.03125

DECISION VALUE: 55
Correct FHC: 40 Incorrect FHC: 9 Accuracy: 0.8163265306122449
TRUE POSITIVE : 31
TRUE NEGATIVE : 9
FALSE POSITIVE : 8
FALSE NEGATIVE  : 1
TRUE POSITIVE RATE : 0.96875
TRUE NEGATIVE RATE : 0.5294117647058824
FALSE POSITIVE RATE : 0.47058823529411764
FALSE NEGATIVE RATE : 0.03125

DECISION VALUE: 60
Correct FHC: 35 Incorrect FHC: 14 Accuracy: 0.7142857142857143
TRUE POSITIVE : 31
TRUE NEGATIVE : 4
FALSE POSITIVE : 13
FALSE NEGATIVE  : 1
TRUE POSITIVE RATE : 0.96875
TRUE NEGATIVE RATE : 0.23529411764705882
FALSE POSITIVE RATE : 0.7647058823529411
FALSE NEGATIVE RATE : 0.03125

